Better Fewer but Better: Community Search with Outliers

Given a set of vertices in a network, that we believe are of interest for the application under analysis, community search is the problem of producing a subgraph potentially explaining the relationships existing among the vertices of interest. In practice this means that the solution should add some vertices to the query ones, so to create a connected subgraph that exhibits some "cohesiveness" property. This problem has received increasing attention in recent years: while several cohesiveness functions have been studied, the bulk of the literature looks for a solution subgraphs containing all the query vertices. However, in many exploratory analyses we might only have a reasonable belief about the vertices of interest: if only one of them is not really related to the others, forcing the solution to include all of them might hide the existence of much more cohesive and meaningful subgraphs, that we could have found by allowing the solution to detect and drop the outlier vertex. In this paper we study the problem of community search with outliers, where we are allowed to drop up to $k$ query vertices, with $k$ being an input parameter. We consider three of the most used measures of cohesiveness: the minimum degree, the diameter of the subgraph and the maximum distance with a query vertex. By optimizing one and using one of the others as a constraint we obtain three optimization problems: we study their hardness and we propose different exact and approximation algorithms.

==> casestudies.tex <==



==> experiments.tex <==
%\note[Lorenzo]{
%	Tipo espetimenti:
%	-real world network
%	-grund truth (dblp)
%	
%	Le dimensioni principali degli esperimenti sono:
%	- Varie misure di qualita' al variare di k
%	- La relazione tra il k in input e il numero vero di outliers trovati (controllando il numero di query node che vengono da comunita’ diverse)
%	- Relazione tra |Q| e k
%	-Relazione diam e |Q|
%	-Relazione diam e mindegree
%	- Confronti con altri metodi(?)
%}
In this section we experimentally evaluate the efficiency and the effectiveness of the community search with outliers. We solve the Community Search with Minimum Diameter, Minimum Degree Constraint and Outliers on some real-world networks in Table~\ref{tab:graphs}.
We perform each experiments 10 times and we report the average value.
All algorithms are implemented in \texttt{C++}, building on the open-source NetworKit framework\footnote{\url{http://networkit.iti.kit.edu/}}.
The experiments are conducted on a server equipped with 64 GB RAM and with a processor Intel 2.4 GHz CPU.\\
\noindent\textbf{Datasets.}
We use four real-world, publicly-available graphs whose characteristics are summarized in Table~\ref{tab:graphs}.
All graphs are undirected and unweighted: \texttt{jazz}\footnote{\url{http://konect.uni-koblenz.de/}\label{footnote:konect}} is a collaboration network among jazz musicians; \texttt{facebook-comb}\footnote{\url{http://snap.stanford.edu/}\label{footnote:snap}} (\texttt{FBco}),
\texttt{soc-youtube}{\ref{footnote:snap}} (	\texttt{sytb}) ,
\texttt{com-amazon}\textsuperscript{\ref{footnote:snap}} (	\texttt{anzb}) is a co-purchasing network and \texttt{dblp2015}\footnote{\url{https://dblp.uni-trier.de/}} (\texttt{dblp}) is a collaboration network crawled in 2015.
\begin{table}[t!]
	%\vspace{-3mm}
	\centering
	\caption{Characteristics of datasets used.}
	\vspace{2mm}
	\label{tab:graphs}
	\small
	%\setlength\tabcolsep{1.8pt}
	\begin{tabular}{r|c|c|c|c|c|}
		
		\multicolumn{1}{c}{}	 & \multicolumn{1}{c}{$|V|$} & \multicolumn{1}{c}{$|E|$} & \multicolumn{1}{c}{avg deg} & \multicolumn{1}{c}{max deg} & \multicolumn{1}{c}{diameter} \\
		\cline{2-6}
	%	\texttt{jazz} & 198 & 2,742  &27.70&100 & 6\\
		\texttt{FBco} & 4,039 & 88,234  &43.69&1,045&8\\
		\texttt{amzn} & 334,863 &925,872  &3.38&549 & 44 \\
		\texttt{com-dblp}&317,080&1,049,866&&&\\
	%	\texttt{sytb} &495,957  &1,936,748   &3.91&25,409&21\\
	%	\texttt{dblp} &1,305,445&6,108,727&9.36 &1,993&23\\
		\cline{2-6}
	\end{tabular}
	\vspace{-3mm}
\end{table}


\noindent\textbf{Query Selection}\\
We use a similar query selection strategy used in~\cite{RuchanskyBGGK17}.
We define different query sets by exploiting the preexisting community structure. In particular, we use three parameters: the number of query vertices, the number of communities they span, and the minimum number of query vertices that should come from the same community. In more details, given a
graph $G=(V,E)$ and a community membership vector $C$, where $C(u)=c_i$, $i$ indicates that vertex $u$ participates in community $i$, we generate a query set $Q$ with three parameters: $n$,$m$, and $k$ by taking the following steps:
(1) select a random community $c_i$;(2)select $n$ vertices that belong to $ci$;(3) select $m$ vertices across $k$ other communities $c_j$,$c_i$. By this construction, we can cover a range of query types. Each experiment is executed 10 times and each value is an average of 10 different experiments.
in the following experiments we choose $|Q|=[20,40]$, $n=[0,20]$ and $m=k=20$.
\subsection{Running time}
In Figure~\ref{Fig:running-time} we report the running time varying the number of outliers some networks in Table~\ref{tab:graphs}. 

We run Algorithm~\ref{alg:mindegree} with $d_{max}=|V|$. We notice that  we can compute the solution in at most 200 second in every network. Moreover, we can see that, if we increase the number of outliers also the running time increases; this is due to the fact that there are more feasible solutions an the algorithm need more iterations to explore all the possible feasible subgraphs.
%\begin{figure}
%\begin{tabular}{cc}
%	\texttt{\texttt{facebook-comb}} & \texttt{com-amazon} \\
%	\hspace{-4mm}\includegraphics[width=.245\textwidth]{{plot/facebook_combined-tab.rt}.pdf}&
%		\hspace{-4mm}\includegraphics[width=.245\textwidth]{{plot/com-amazon.ungraph.rt}.pdf}\\
%		\multicolumn{2}{c}{\texttt{com-dblp}}\\
%\multicolumn{2}{c}{\hspace{-4mm}\includegraphics[width=.245\textwidth]{{plot/com-dblp.ungraph.rt}.pdf}}\end{tabular}
%\vspace{-2mm}
%\caption{Running time of Algorithm~\ref{alg:mindegree} with $d_{max}=|V|$ on some networks in Table~\ref{tab:graphs}.}
%\label{Fig:running-time}
%%\vspace{-3mm}
%\end{figure}

\subsection{Studying the quality of the solution}
\note[Lorenzo]{add plots and comments}
%\noindent\textbf{Studying the query selection}\\
\noindent\textbf{Varying the number of outliers} We measure the characteristics of the solution varying the number of outliers. We run Algorithm~\ref{alg:mindegree} with $d_{max}=|V|$.In Figure~\ref{Fig:vh} we report the the size of the solution $|H|$: we can see that increasing the number of outliers, the number of vertices in the solution decrease. Also the Diameter of $|H|$ (Figure~\ref{Fig:diameter}) decreases allowing more outliers in the solution. We report also the effective number of query nodes in Figure~\ref{Fig:qh} and the minimum degree among all the vertices in the solution (Figure~\ref{Fig:mindegree}): allowing the possibility to discard some query node improve the minimum maximum degree in $H$
\begin{figure}
	\begin{tabular}{ccc}
		\texttt{\texttt{facebook-comb}} & \texttt{com-amazon}&{\texttt{com-dblp}} \\
		\hspace{-4mm}\includegraphics[width=.16\textwidth]{{plot/facebook_combined-tab.diameter}.pdf}&
		\hspace{-4mm}\includegraphics[width=.16\textwidth]{{plot/com-dblp.ungraph.diameter}.pdf}&{\hspace{-4mm}\includegraphics[width=.16\textwidth]{{plot/com-dblp.ungraph.diameter}.pdf}}\\
	\end{tabular}
	\vspace{-2mm}
	\caption{Diameter of the subgraph returned by Algorithm~\ref{alg:mindegree} with minimum degree on some networks in Table~\ref{tab:graphs}.}
	\label{Fig:diameter}
	%\vspace{-3mm}
\end{figure}
\begin{figure}
	\begin{tabular}{cc}

		\texttt{\texttt{facebook-comb}} & \texttt{com-amazon} \\
		\hspace{-4mm}\includegraphics[width=.245\textwidth]{{plot/facebook_combined-tab.mindeg}.pdf}&
		\hspace{-4mm}\includegraphics[width=.245\textwidth]{{plot/com-amazon.ungraph.mindeg}.pdf}\\
					\multicolumn{2}{c}{\texttt{com-dblp}}\\
	\multicolumn{2}{c}{\hspace{-4mm}\includegraphics[width=.245\textwidth]{{plot/com-dblp.ungraph.mindeg}.pdf}}\\
	\end{tabular}
	\vspace{-2mm}
	\caption{{Minimum degree of the subgraph returned by Algorithm~\ref{alg:mindegree} with minimum degree on some networks in Table~\ref{tab:graphs}.}}
	\label{Fig:mindegree}
	%\vspace{-3mm}
\end{figure}

\begin{figure}
	\begin{tabular}{cc}
		\texttt{\texttt{facebook-comb}} & \texttt{com-amazon}\\
		\hspace{-4mm}\includegraphics[width=.245\textwidth]{{plot/facebook_combined-tab.qh}.pdf}&
		\hspace{-4mm}\includegraphics[width=.245\textwidth]{{plot/com-amazon.ungraph.qh}.pdf}\\
					\multicolumn{2}{c}{\texttt{com-dblp}} \\
		\multicolumn{2}{c}{\hspace{-4mm}\includegraphics[width=.245\textwidth]{{plot/com-dblp.ungraph.qh}.pdf}}\\
	\end{tabular}
	\vspace{-2mm}
	\caption{Effective number of query nodes ($|Q_H$) in the subgraph returned by Algorithm~\ref{alg:mindegree} with minimum degree on some networks in Table~\ref{tab:graphs}.}
	\label{Fig:qh}
	%\vspace{-3mm}
\end{figure}
\begin{figure}
	\begin{tabular}{cc}
		\texttt{\texttt{facebook-comb}} & \texttt{com-amazon}\\
		\hspace{-4mm}\includegraphics[width=.245\textwidth]{{plot/facebook_combined-tab.vh}.pdf}&
		\hspace{-4mm}\includegraphics[width=.245\textwidth]{{plot/com-amazon.ungraph.vh}.pdf}\\
		\multicolumn{2}{c}{\texttt{com-dblp}}\\
		\multicolumn{2}{c}{\hspace{-4mm}\includegraphics[width=.245\textwidth]{{plot/com-dblp.ungraph.vh}.pdf}}\\
	\end{tabular}
	\vspace{-2mm}
	\caption{Size of the subgraph returned by Algorithm~\ref{alg:mindegree} with minimum degree on some networks in Table~\ref{tab:graphs}.}
	\label{Fig:vh}
	%\vspace{-3mm}
\end{figure}
%\noindent\textbf{Varying the maximum minimum degree}\\

\noindent\textbf{Varying the distance constraint} 
We................
\begin{figure}
	\begin{tabular}{cc}
		
		\texttt{\texttt{soc-youtube}} & \texttt{soc-youtube} \\
		\hspace{-4mm}\includegraphics[width=.245\textwidth]{{plot/com-youtube.ungraph.dist.mindeg}.pdf}&
		\hspace{-4mm}\includegraphics[width=.245\textwidth]{{plot/com-youtube.ungraph.dist.vh}.pdf}\\
	
	\end{tabular}
	\vspace{-2mm}
	\caption{{Minimum degree of the subgraph returned by Algorithm~\ref{alg:mindegree} with minimum degree on some networks in Table~\ref{tab:graphs}.}}
	\label{Fig:mindegree}
	%\vspace{-3mm}
\end{figure}
%We measure the diameter, the size of the subgraph $H$ and the clustering coefficient varying the distance constraint in Algorithm~\ref{alg:mindegree}:
%\begin{figure}
%	\begin{tabular}{cc}
%	\texttt{com-amazon} & \texttt{com-amazon} \\
%		\hspace{-4mm}\includegraphics[width=.245\textwidth]{{plot/com-amazon.ungraph.md.diam}.pdf}&
%		\hspace{-4mm}\includegraphics[width=.245\textwidth]{{plot/com-amazon.ungraph.md.cc}.pdf}\\
%		\multicolumn{2}{c}{\texttt{com-amazon}} \\
%		\multicolumn{2}{c}{\hspace{-4mm}\includegraphics[width=.245\textwidth]{{plot/com-amazon.ungraph.md.vh}.pdf}}\\
%	\end{tabular}
%	\vspace{-2mm}
%	\caption{cc}
%	\label{Fig:md}
%	%\vspace{-3mm}
%\end{figure}
%\begin{figure}
%	\begin{tabular}{cc}
%		\texttt{--} & \texttt{--} \\
%		\hspace{-4mm}\includegraphics[width=.245\textwidth]{{plot/com-youtube.ungraph.rt}.pdf}&
%		\hspace{-4mm}\includegraphics[width=.245\textwidth]{{plot/com-youtube.ungraph.rt}.pdf}\\
%	\end{tabular}
%	\vspace{-2mm}
%	\caption{-.}
%	\label{Fig:running-time}
%	%\vspace{-3mm}
%\end{figure}
\subsection{Case of study: DBLP}
\texttt{dblp2015} is a collaboration network where each vertex represents an author and an edge between two authors means that they have co-authored a paper. The details of the network are reported in Table~\ref{tab:graphs}.
We use the query set $Q=\{Kleinberg,Raghavan,Gionis,Aceto\}$ where the first three authors are researchers the data mining area while the latter is a researcher in formal methods. We run the experiments with distance constraints equal to 2, since we want to include only authors that have at least a common co-author with $Q$. We varying the number of outliers up to 2 and we report in Table~\ref{tab:dblp} the characteristics of the solutions. We notice that that allowing one or two outliers, the vertex \emph{Aceto}, the only one not belonging to the data mining community, is removed from the solution. Moreover Algorithm~\ref{} returns a subgraph $H$ smaller and with higher clustering coefficient than the solution with no outliers. 
\begin{table}[t!]
	%\vspace{-3mm}
	\centering
	\caption{Solution of the query set $Q=\{Kleinberg,Raghavan,Gionis,Aceto\}$ in the \texttt{dblp2015} collaboration network with different number of outliers. }
	\vspace{2mm}
	\label{tab:dblp}
	\small
	%\setlength\tabcolsep{1.8pt}
	\begin{tabular}{r|c|c|c|c|c|}
		
		\multicolumn{1}{c}{}	 & \multicolumn{1}{c}{$k$} & \multicolumn{1}{c}{$|H|$} & \multicolumn{1}{c}{$D$} & \multicolumn{1}{c}{$Q_H$} & \multicolumn{1}{c}{CC} \\
		\cline{2-6}
 &0&3942&6&4&0.32\\
 &[1,2]&1512&5&3&0.47\\

		\cline{2-6}
	\end{tabular}
	\vspace{-3mm}
\end{table}






==> multicomm.tex <==
Sometimes the query nodes may belong to different communities: we extend the definitions of the problems in Section~\ref{sec:problem} in order to identify multiple connectors containing at least $\ell$ vertices, where $\ell$ is an input parameter. \note[lorenzo]{We consider not overlapping communities}
%We consider non-overlapping connectors.

\begin{problem} \label{prob:min_deg:multi}
	%	\noindent \textbf{Community Search with Maximum Minimum Degree, Max Diameter Constraint and Outliers (CSMaxDegDiamO)}
	Given a graph $G=(V_G,E_G)$, a set of query vertices $Q \subseteq V_G$, an integer $0\leq \ell \leq |Q|$, an integer $diam_{\max} \geq 1$,   find a set $\mathcal{H}$ of induced subgraphs $H=(V_H,E_H)$ of $G$  such that:
	
	\begin{enumerate}
		\item $\forall H\in \mathcal{H}$, $H$ is connected;
				\item $\forall H',H''\in \mathcal{H}$, $V_{H'}\cap V_{H''} =\emptyset$;
		\item  $\forall H\in \mathcal{H}$ , $|V_H \cap Q| \geq \ell$;
		\item $\forall H\in \mathcal{H}$ ,$diam(H) \leq diam_{\max}$
		\item $\forall H\in \mathcal{H}$, the minimum degree if $H$ is maximized among all subgraphs satisfying 1-4 and containing $V_H\cap Q$;
	\end{enumerate}
\end{problem}
\begin{problem}\label{prob:min_deg2:multi}
%	\note[lorenzo]{I think it is the hardest problem...}
	%\noindent \textbf{Community Search with Maximum Minimum Degree, Max Distance Constraint and Outliers (CSMaxDegDistO)}
	Given a graph $G=(V_G,E_G)$, a set of query nodes $Q \subseteq V_G$, an integer $0\leq \ell \leq |Q|$, an integer $d\geq1$,  find a set $\mathcal{H}$ of induced subgraphs $H=(V_H,E_H)$ of $G$  such that:
	
	\begin{enumerate}
		
		\item $\forall H\in \mathcal{H}$, $H$ is connected;
				\item $\forall H',H''\in \mathcal{H}$, $V_{H'}\cap V_{H''} =\emptyset$;
		\item  $\forall H\in \mathcal{H}$ , $|V_H \cap Q| \geq \ell$;
		\item $\forall H\in \mathcal{H}$ , for any node $v \in V_H$, $d(Q,v) := \min_{q \in V_H \cap Q} d(q,v) \leq d$
		\item $\forall H\in \mathcal{H}$, the minimum degree if $H$ is maximized among all subgraphs satisfying 1-4 and containing $V_H\cap Q$;


	\end{enumerate}
\end{problem}
\begin{problem}\label{prob:min_dia:multi}
	%	\noindent \textbf{Community Search with Minimum Diameter, Minimum Degree Constraint and Outliers (CSMinDiamDegO)}
	Given a graph $G=(V_G,E_G)$, a set of query nodes $Q \subseteq V_G$, an integer $0\leq \ell \leq |Q|$, an integer $\delta_{\min} \geq 0$,find a set $\mathcal{H}$ of induced subgraphs $H=(V_H,E_H)$ of $G$  such that:
	
	\begin{enumerate}
			\item $\forall H\in \mathcal{H}$, $H$ is connected;
				\item $\forall H',H''\in \mathcal{H}$, $V_{H'}\cap V_{H''} =\emptyset$;
		\item  $\forall H\in \mathcal{H}$ , $|V_H \cap Q| \geq \ell$;
		\item $\forall H\in \mathcal{H}$ ,the minimum degree in $H$ is at least $\delta_{\min}$;
		\item $\forall H\in \mathcal{H}$, $diam(H)$ is minimized among all subgraphs satisfying 1-4 and containing $V_H\cap Q$;

	\end{enumerate}
\end{problem}
